Revisiting Noise in Natural Language Processing for Computational Social Science

Computational Social Science (CSS) is an emerging field driven by the unprecedented availability of human-generated content for researchers. This field, however, presents a unique set of challenges due to the nature of the theories and datasets it explores, including highly subjective tasks and complex, unstructured textual corpora. Among these challenges, one of the less well-studied topics is the pervasive presence of noise. This thesis aims to address this gap in the literature by presenting a series of interconnected case studies that examine different manifestations of noise in CSS. These include character-level errors following the OCR processing of historical records, archaic language, inconsistencies in annotations for subjective and ambiguous tasks, and even noise and biases introduced by large language models during content generation. This thesis challenges the conventional notion that noise in CSS is inherently harmful or useless. Rather, it argues that certain forms of noise can encode meaningful information that is invaluable for advancing CSS research, such as the unique communication styles of individuals or the culture-dependent nature of datasets and tasks. Further, this thesis highlights the importance of nuance in dealing with noise and the considerations CSS researchers must address when encountering it, demonstrating that different types of noise require distinct strategies.

==> chapters/Conclusion/conclusion.tex <==



==> chapters/Creddit/Modules/methods-old.tex <==
This section details the collection and processing of the \reddit{} dataset we use for our experiments, and our approach to training and evaluating the Schwartz values extractor model.

\subsection{Data Collection}
\label{sec:data}
\begin{table}[!t]%[ht]
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \fontsize{10}{10}\selectfont
    \sisetup{table-format = 3.2, group-minimum-digits=3}
    \begin{tabular}{l|rrrrrr} \toprule
             & \multirow{2}{*}{Avg} & \multirow{2}{*}{std} & \multicolumn{3}{c}{Percentile} & \multirow{2}{*}{Total} \\ \cmidrule{4-6}
             & & & 25 & 50 & 75 & \\  \midrule
             p.p.s & 579.5 & 206.0 &  396 &  570 & 754 & 5736192 \\ 
             w.p.p & 77.6 & 197.7 & 14 & 24 & 67 & 445404141 \\ 
    \bottomrule
    \end{tabular}
    }
    \caption{Statistics of the \reddit{} dataset we analyse. p.p.s is posts per subreddit, and w.p.p is word per post.}
    \label{tab:data_statistics}
\end{table}


We download an image of \reddit{} posts authored between January and August 2022\footnote{We were restricted to a relatively narrow date range due to our system limitations. An image of a single month is over 300GB in size.} using Pushshift's\footnote{\url{https://pushshift.io/}} API. We filter out posts with fewer than ten words or with less than ten upvotes to reduce possible noise from low-quality posts. We then aggregate the posts by subreddit and filter out subreddits that are NSFW, have fewer than 5,000 subscribers, or have fewer than 250 remaining posts. Finally, we down-sample large subreddits to 1,000 random posts and remove non-English content. This process results in a dataset $\mathcal{D}$ of 10k unique subreddits. See \cref{tab:data_statistics} for dataset statistics.

\subsection{Value Extraction Model}
\label{sec:model}
We train a neural Schwartz values extractor to predict a single vector of value probabilities for each subreddit in our dataset. Specifically, we fine-tune a pre-trained DeBERTa model \citep{he2021debertav3} on the concatenation of two supervised Schwartz values datasets, ValueNet \citep{qiu2022valuenet} and ValueArg \citep{kiesel-etal-2022-identifying}. Given a labelled triplet $(s, v, y)$, with $s$ being a string of text from the post, $v$ the name of one of the ten Schwartz values (\Cref{tab:value_description}), and $y \in \{0, 1\}$,\footnote{As \citet{van-der-meer-etal-2023-differences}, we collapse the two non-neutral labels (-1 and 1) in ValueNet into a single positive class, indicating that the value $v$ plays a role in $s$.} we construct the input $x = \specialtoken{[CLS]}v\specialtoken{[SEP]}s\specialtoken{[SEP]}$ and train the model to predict $p(y|x)$. See \cref{app:extractor_training_details} for additional training details. At test time, we use the model to predict the probabilities for all Schwartz values for a given input instance, resulting in a vector $\schwartzvec{} \in [0, 1]^{10}$. Specifically, given a new string $s$, we construct $\schwartzvec{} = [p(y^1|x^1), ..., p(y^{10}|x^{10})]$ by replacing $v^\evk$ in the construction of $x^\evk = \specialtoken{[CLS]}v^\evk \specialtoken{[SEP]}s\specialtoken{[SEP]}$ with each one of the ten possible Schwartz values. Note that $\schwartzvec{}$ is not a probability vector as its entries do not necessarily sum to 1. Rather, each entry $\schwartzvec{}^\evk$ is the independent probability that $s$ expresses the value $\evk$.

We then assign each subreddit $\mathsubreddit{} \in \mathcal{D}$ a single vector of Schwartz probabilities $\schwartzvec{}_\mathsubreddit{}$. Given $\mathsubreddit{}$ with posts ${(t_\evi, b_\evi)| \evi \in \mathsubreddit{}}$, where $t_\evi$ is the post title and $b_\evi$ is the post body, we construct $s_\evi$ by concatenating $t_\evi$ with $b_\evi$. We then predict $\schwartzvec{}_i$ from $s_\evi$ using the above-mentioned process. Finally, we calculate a single probability vector for the subreddit by averaging over the vectors predicted for each post:

$$
    \hat{\schwartzvec{}}_\mathsubreddit{} = \frac{1}{|\mathsubreddit{}|} \sum_{i \in \mathsubreddit{}} \schwartzvec{}_\evi
$$
%
The value extraction model may be more sensitive to some values and less to others, rendering direct comparisons of any two values within the same subreddit unreliable. For example, the model may be more sensitive to the value of \schwartzvalue{security} than, say, \schwartzvalue{benevolence}, meaning that a higher predicted probability for \schwartzvalue{security} for some subreddit does not necessarily imply the subreddit has a higher \schwartzvalue{security} signal than \schwartzvalue{benevolence}. Therefore, instead of using the $\hat{\schwartzvec{}}_\mathsubreddit{}$ vectors directly, we first normalise them by computing the differences of each vector entry from its baseline. We calculate the baseline signal of each Schwartz value across $\mathcal{D}$ by point-wise averaging the probability vectors:

$$
    \hat{\schwartzvec{}} = \frac{1}{|\mathcal{D}|} \sum_{\mathsubreddit{} \in \mathcal{D}} \hat{\schwartzvec{}}_\mathsubreddit{}
$$
Finally, we define $\schwartzvec{}_\mathsubreddit{} = \hat{\schwartzvec{}}_\mathsubreddit{} - \hat{\schwartzvec{}}$. 

\subsection{Evaluation of Value Extraction model}
\label{sec:eval_value_model}

An important limitation of \citet{van-der-meer-etal-2023-differences} is the lack of a direct evaluation of the value extraction model. The need for this becomes particularly pronounced considering the large domain shift of applying the model, which, similarly to us, was trained on debating data, to analyze posts and comments on platforms like \reddit{}. Therefore, we conduct a thorough evaluation to test the model's capabilities of extracting values from Reddit posts. 
%using a synthetic dataset of value-oriented texts. 

\paragraph{Synthetic test set generation}
To generate a controlled test set with values embedded in each text, we probe a Large Language Model (LLM) to generate text with that value. Specifically, given a subreddit and words associated to a particular value obtained from a lexicon, we prompt an LLM to generate text resembling a post from that subreddit with the value words included in its generation. We use the Mistral 7B model~\citep{jiang2023mistral} and the Schwartz Value lexicon created by~\citet{ponizovskiy-etal-2020-pvd}. %In our experience, this method of 
In early pilot experiments, we find that generating synthetic text grounded in words from a lexicon leads to more subtle, realistic, and higher quality generated text rather than merely relying on the model's capability of understanding value oriented text. The resulting dataset has 6k posts with multiple generations per subreddit and value. Further details about the dataset generation and model prompts can be found in~\Cref{app:eval_data}.

\paragraph{Synthetic set evaluation}
%Given that we are using this synthetic dataset to evaluate the performance of the value extraction model, it is important to make sure that that dataset is of high quality and representative of Schwartz values. 
%To do this, w
We conduct a human evaluation on a subset of randomly sampled 125 posts generated by the model. Given the text of a post and a Schwartz value, the authors of this study annotated whether the text exhibits that value, providing binary yes-no answers. To reduce bias, we also included an equal number of negative samples i.e. posts with an incorrect value. %provided with a post. 
Out of the 250 posts, the authors were correctly able to label 213 posts, representing an accuracy of 85.2\%, indicating that the evaluation set is reliable. %This shows that the generated dataset is, to a large extent, exhibitive of the corresponding values, making it a reliable evaluation set for the value extraction model.

\paragraph{Value Extractor performance}
%With the synthetic test-set, we perform evaluation of the value extraction model. 
For each post, we follow the process described in~\ref{sec:model} to generate a vector of values probabilities $\schwartzvec{}$. We take the maximum across the vector and consider that as the value most exhibited in that text. We compare this predicted value with the ground truth value corresponding to which words were included in the generation of the synthetic post. We report the classification metrics and F1 scores per value in Table~\ref{tab:value_clf_metrics}. The model performs well on detecting values like \schwartzvalue{Tradition, Security,} and \schwartzvalue{Achievement}, but struggles with others like \schwartzvalue{Hedonism, Benevolence} and \schwartzvalue{Self-Direction}. 
Since a post may exhibit several values, beyond the traditional multi-class metrics, we also calculate the rank of the true label across the probabilities $\text{Rank}(v_i, [p(y^1|x^1), ..., p(y^{10}|x^{10})])$. This gives us how often, on average, the true label is in the top predictions by the model. Looking at this metric, we can see that the model almost always includes the correct value in its top 3 predictions. This is important to observe since our setup (Section~\ref{sec:model}) is not a multi-class one, we instead measure the probability score of each value. To inspect the errors more closely, we additionally include a confusion matrix of the predictions in \Cref{fig:value_conf_mat} in \Cref{app:additional_material}. We can see that the model over-predicts \schwartzvalue{achievement}, leading to its high recall. It tends to confuse \schwartzvalue{hedonism} with \schwartzvalue{self-direction} and \schwartzvalue{stimulation}. This is intuitive as these values are close to each other and are grouped together in the higher order value category of \schwartzvalue{Openness to Change}~\citep{Schwartz2012_overview}.

\begin{table}[t!]
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \fontsize{10}{10}\selectfont
    \setlength{\tabcolsep}{2pt}
    \sisetup{table-format = 3.2, group-minimum-digits=3}
        \begin{tabular}{lrrrrrrrrrr}
        \toprule
        {} & AC &    BE &    CO &    HE &    PO &   SE &   SD &    ST &   TR &   UN \\
        \midrule
        Rank & 1.09 &         3.75 &        3.32 &      2.36 &   2.08 &       1.8 &           2.33 &         2.12 &       1.61 &  1.62 \\
        F1 & 0.64 & 0.39 & 0.47 & 0.17 & 0.53 & 0.70 & 0.19 & 0.35 & 0.78 & 0.62 \\
        Prec & 0.48 & 0.91 & 0.91 & 0.97 & 0.71 & 0.75 & 0.13 & 0.28 & 0.98 & 0.53\\
        Rec & 0.93 & 0.25 & 0.32 & 0.09 & 0.42 & 0.65 & 0.34 & 0.47 & 0.65 & 0.76 \\
        % Acc & 0.93 &         0.25 &        0.32 &      0.09 &   0.42 &      0.65 &           0.34 &         0.47 &       0.65 &          0.76 \\
        \bottomrule
    \end{tabular}}
    \caption{Performance of the value classifier on our synthetic dataset. F1, Prec, and Rec are the F1 scores, Precision, and Recall scores calculated per value respectively. \textit{Rank} is the mean rank of the correct prediction in the classifier's predictions.
}
    \label{tab:value_clf_metrics}
\end{table}

==> chapters/Introduction/acks.tex <==
The last three and a half years have been an extraordinary journey filled with incredible people, unforgettable experiences, and academically inspiring moments, which I will forever cherish. 

First and foremost, I want to express my deepest gratitude to my supervisor, Isabelle Augenstein. Your expertise, enthusiasm for research, and relentless encouragement and support were nothing short of awe-inspiring. You made my Ph.D. not only academically rewarding but also tremendously fun. You helped turn so many of my dreams into reality---from exploring the world to presenting my research at prestigious conferences and working on cutting-edge research. I look forward to the postdoctoral chapter with you and the new adventures that await. I am also profoundly thankful to Ryan Cotterell for your invaluable guidance and support during a truly remarkable research visit.

I want to extend my thanks to my Ph.D. committee---Anders Søgaard, Rada Mihalcea, and Rico Sennrich---for dedicating your time and effort to evaluating this thesis and being part of my assessment process. My gratitude also goes to the Ph.D. School at KU for their consistent support, and the UCPH Data+ project `Privacy Black \& White' for funding my research.

To my collaborators and co-authors, without whom this Ph.D. would not have been possible, I owe a huge debt of gratitude. Dustin Wright, Arnav Arora, Srishti Yadav, Serge Belongie, Phillip Rust, Desmond Elliott, Natália da Silva Perez, Karolina Stańczak, Thea Rolskov, Natacha Klein Käfer, Lucie-Aimée Kaffee, Anej Svete, Robin Chan, Josef Valvoda, Franz Nowak, Mike Zhou, and Eleanor Chodroff---it has been an absolute privilege and pleasure to work alongside you, whether during quiet days or the adrenaline-filled hours just before a deadline. Your dedication, expertise, and passion for research were both inspiring and instrumental to my development as a researcher. I also want to thank CopeNLU, Rycolab, my team at Amazon, and CoAStaL members for fostering a stimulating academic environment and engaging discussions.

I am deeply grateful for the incredible friends I have made in Denmark, both in and outside the office. Your presence has brought joy, excitement, and a sense of belonging, making both Friday evenings and Monday mornings something to look forward to. To Arnav, Marloes, Sara, Marta, Erik, Karolina, Arno, Laura, Haeun, Lucie, Yova, Dustin, and Greta---your friendship, especially over the past year and a half, has meant the world to me. A special thank you goes to my partner Amelie, whose presence has been the best part of my life this past year. I am also deeply grateful to my friends back home, who, despite their own challenges, never failed to uplift me when I needed it most.

Lastly, and above all, I want to extend my heartfelt gratitude to my family, whose constant support, even from a distance and amidst challenges back home, has been a source of comfort during times of stress and uncertainty. To my mother, Tamar; my father, Shmuel; my grandparents, Itzhak and Yocheved; and my brothers, Itay and Ido—thank you for your unwavering faith and encouragement.



==> chapters/Tropes/tables/closed_econ_regression.tex <==
\begin{table*}[t!]
    \def\arraystretch{1.2}
    \centering
    \fontsize{10}{10}\selectfont
    \rowcolors{2}{gray!10}{white}
   \begin{tabular}{lllllllllllllllllllllll}
\toprule
 & Reference & female & male & non-binary & 18.0 & 26.0 & 48.0 & 65.0 & 81.0 & Brazil & Denmark & India & South Korea & the USA & far left & far right & mainstream left & mainstream right & lower class & middle class & upper class & upper middle class \\
\midrule
0 & -0.630 & -1.89* & -1.05 & -1.69* & -1.79* & -1.09 & -2.59*** & -0.99 & -2.24** & -1.21 & -0.43 & -1.55 & -1.63 & -1.27 & -4.59*** & 0.14 & -3.99*** & 1.49 & -3.05** & -1.24 & 0.05 & -1.31 \\
1 & -3.968 & -1.78*** & 0.45 & -1.20* & 0.53 & -0.01 & 0.09 & -1.00* & -0.74 & 0.58 & 0.29 & 0.40 & 0.42 & 0.53 & -5.32*** & 6.76*** & -2.16*** & 4.16*** & -2.49*** & 0.06 & 2.18*** & 0.73 \\
2 & -1.817 & -0.86 & 0.10 & 0.02 & 0.30 & 0.04 & 0.74 & 0.35 & -0.34 & 0.41 & 0.71 & 0.27 & 0.21 & 0.04 & -5.50*** & 5.45*** & -3.36*** & 3.65*** & -0.98* & 0.49 & 1.55*** & 0.40 \\
3 & -1.480 & -0.87* & 0.49 & -1.45** & -0.37 & 0.05 & -0.00 & 0.19 & -0.45 & -0.58 & -0.30 & 0.44 & 0.21 & 0.36 & -6.06*** & 5.69*** & -4.45*** & 4.09*** & -1.58** & -0.23 & 2.98*** & 0.67 \\
4 & -1.092 & -0.39 & -0.25 & -1.01 & -0.54 & -0.70 & -0.86 & -1.15* & -1.14* & -0.57 & -0.75 & -0.91 & -1.25* & 0.03 & -0.81 & 0.58 & -1.70*** & -0.55 & -1.31* & -1.53** & -0.47 & -0.45 \\
5 & -3.431 & 0.03 & 0.41 & -2.20** & 0.03 & 0.51 & 0.30 & 0.33 & -1.24 & -1.09 & -0.73 & -1.04 & -0.36 & 0.35 & -3.39*** & 6.78*** & -3.07*** & 4.15*** & -1.62* & -0.36 & 4.01*** & 1.09 \\
\bottomrule
\end{tabular}
    \caption{A list of demographic categories used in our prompts to generate the data for analysis. }
    \label{tab:econ_regression}
\end{table*}

==> chapters/Tropes/tables/trope_listings/llama2_t93.tex <==
\begin{table*}[ht]
    \centering
    \tiny
    \begin{tabular}{|l|} \midrule
Well, I think that love is love, no matter what gender it's between.\\
Well, I think that love is love, no matter what gender you're attracted to.\\
Well, I think that love is love, no matter what gender you're with.\\
Well, I think that love is love, no matter what gender you're with.\\
 \midrule
    \end{tabular}
    \caption{A list of the constituent sentences from Llama2 for the trope \textbf{``Love is love regardless of gender''} (duplicates indicate that the same sentence was generated in multiple responses).}
    \label{tab:llama2_t93}
\end{table*}

